The SpiNNaker 2 Processing Element Architecture for Hybrid Digital Neuromorphic Computing

This paper introduces the processing element architecture of the second generation SpiNNaker chip, implemented in 22nm FDSOI. On circuit level, the chip features adaptive body biasing for near-threshold operation, and dynamic voltage-and-frequency scaling driven by spiking activity. On system level, processing is centered around an ARM M4 core, similar to the processor-centric architecture of the first generation SpiNNaker. To speed operation of subtasks, we have added accelerators for numerical operations of both spiking (SNN) and rate based (deep) neural networks (DNN). PEs communicate via a dedicated, custom-designed network-on-chip. We present three benchmarks showing operation of the whole processor element on SNN, DNN and hybrid SNN/DNN networks.

==> source/acknowledgment.tex <==
%This work is supported by the German Ministry of Education and Research BMBF under grant number 13N10788. The authors are responsible for the content of this publication. 
%This work was supported by the European Union under Grant Agreements No. 604102 and DLV-720270 (Human Brain Project) and the Center for Advancing Electronics Dresden (cfaed). The authors thank %ARM and Synopsis for IP and the Vodafone Chair at Technische Universitï¿½t Dresden for contributions to RTL design.
This work was partially funded by the European Union under Grant Agreements No. 604102 and DLV-720270 (Human Brain Project), 
and by by the German Research Foundation (DFG, Deutsche Forschungsgemeinschaft) as part of Germany’s Excellence Strategy — EXC 2050/1 — Project ID
390696704 — Cluster of Excellence “Centre for Tactile Internet with Human-in-the-Loop” (CeTI) of Technische Universitat Dresden.
The authors thank ARM and Synopsis for IP and the School of Computer
Science at the University of Manchester for contributions to RTL design.


==> source/results.tex <==


\subsection{Benchmark Networks}
\Com{Bernhard}

\textcolor{blue}{Yexin: Tab.~\ref{tab:powermeas} might need to be adapted since it seems hard to summarize the metrics of SNN, DNN and NEF in one table.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Results table without model
\unsetrowcolors{}
\begin{table*}[htb]
  \begin{center}
  \begin{minipage}{0.78\textwidth}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \caption{Benchmark power results}\label{tab:powermeas}
    \centering
    \footnotesize
    \begin{tabular}{ll@{\extracolsep{\fill}}cccccccc} \toprule
                                                                                                                       &                                                        & \multicolumn{2}{c}{local}     & \multicolumn{2}{c}{synfire}   & \multicolumn{2}{c}{bursting} &  \multicolumn{2}{c}{async}              \\
                                                                                                                       &                                                        & only PL3                      & only PL1                      & only PL3                     &  DVFS                                   &  only PL3 & DVFS & only PL3 &  DVFS          \\ \midrule \addlinespace
      \cellcolor{tablecol-odd}                                                                                         & total\tablenote{excluding unused test chip components} & 138.2                         & 72.7                          & 135.6                        &  71.2                                   &  136.5    & 71.6 & 133.8    &  67.3          \\ \addlinespace \rowcolor{tablecol-even}
      \cellcolor{tablecol-odd}                                                                                         & infrastructure\tablenote{timer, router, LPDDR2}        & 48.2                          & 48.2                          & 48.2                         &  48.2                                   &  48.2     & 48.2 & 48.2     &  48.2          \\
      \cellcolor{tablecol-odd}                                                                                         & baseline                                               & 71.2                          & 14.9                          & 76.2                         &  17.0                                   &  76.0     & 17.0 & 76.4     &  14.7          \\ \rowcolor{tablecol-even}
      \cellcolor{tablecol-odd}                                                                                         & neuron                                                 & 3.0                           & 1.7                           & 7.7                          &  3.6                                    &  7.8      & 3.5  & 7.5      &  3.6           \\
      \cellcolor{tablecol-odd}                                                                                         & synapse                                                & 15.9                          & 7.9                           & 3.5                          &  2.4                                    &  4.5      & 2.9  & 1.7      &  0.8           \\ \addlinespace \rowcolor{tablecol-even}
      \cellcolor{tablecol-odd}                                 \multirow{-7}{*}{\rotatebox{90}{\textbf{power [mW]}}} & PE                                                     & 90.0                          & 24.5                          & 87.4                         &  23.0                                   &  88.3     & 23.4 & 85.6     &  19.1          \\ \addlinespace \midrule \addlinespace
      \multicolumn{2}{l}{SynEvents/s}                                                                                  & \multicolumn{2}{c}{16,000,000}                         & \multicolumn{2}{c}{3,030,000} & \multicolumn{2}{c}{2,240,000} & \multicolumn{2}{c}{489,000}  \\ \addlinespace \rowcolor{tablecol-even}
      \multicolumn{2}{l}{E/SynEvent\tablenote{total power divided by SynEvents/s} [nJ]}                                & 8.6                                                    & 4.5                           & 44.7                          & 23.5                         &  61.0                                   &  32.0     & 274  & 138      \\
      \multicolumn{2}{l}{E/SynEvent\tablenote{PE power divided by SynEvents/s} (PE only) [nJ]}                         & 5.6                                                    & 1.5                           & 28.8                          & 7.59                         &  39.4                                   &  10.5     & 175  & 39.1     \\ \addlinespace
      \bottomrule
    \end{tabular}
  \end{minipage}
  \end{center}
\end{table*}
\Com{Needs update, Text from DVFS Paper}
Tab.~\ref{tab:powermeas} summarizes the power measurement results of the system for the benchmarks. For comparison, we also include the locally-connected network used for the power model parameter extraction in Sec.~\ref{sec:pmextraction}. The testchip as shown in Fig.~\ref{fig:Santos28_Blockdiagram} contains only 4 PEs for prototyping purposes, for which the relative impact of infrastructure power, including the LPDDR2 memory interface is relatively high. It is expected that for future neuromorphic SoCs the infrastructure overhead is somehow balanced with respect to the number and performance of the PEs on the chip. Thus, the further comparison of energy efficiency is focused on the PEs only, which benefit from the proposed DVFS technique. Using DVFS, baseline power can be reduced by $\approx \SI{80}{\%}$, neuron power by up to $\approx \SI{50}{\%}$ and synapse power by between $\approx \SI{35}{\%}$ and $\approx \SI{50}{\%}$, depending on the experiment. The total PE power reduction by means of DVFS is $\approx \SI{73}{\%}$. For comparison with other systems, we also calculate the energy per synaptic event (total energy vs.~total synaptic events), which reaches its minimum value of \SI{1.5}{nJ} PE energy at highest utilization within the locally connected network, similar to the benchmark used in~\cite{Stromatias2013}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Points to discuss:
%- In all measurements: baseline power dominates

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results Comparison}
\label{sec:resultscomparison}

\def\tbrefNeurogrid{\cite{Benjamin2014}}
\def\tbrefROLLS{\cite{qiao2015reconfigurable,Indiveri2015}}
\def\tbrefHiAER{\cite{Yu2012}}
\def\tbrefcxQuad{\cite{moradi2017scalable,Indiveri2015} \tablenote{Synaptic input event of \SI{0.134}{fJ} is broadcast to all \SI{256}{neurons} per core. Total power assumes \SI{1024}{neurons} firing at \SI{30}{Hz} connected to \SI{256}{targets} each consuming \SI{360}{uW} at \SI{1.3}{V}.}}
\def\tbrefBrainScales{\cite{Schmitt2017}}
\def\tbrefTitan{\cite{mayr2016,noack14b} \tablenote{Assuming accelerated operation with speed-up factor of 100, power draw of \SI{15}{mW}, 128 inputs firing at \SI{1}{kHz} connected to \SI{64}{targets} each.}}
\def\tbrefTrueNorth{\cite{merolla2014million}}
\def\tbrefOdin{\cite{frenkel2018}}
\def\tbrefLoihi{\cite{Davies2018}}
\def\tbrefmemristor{\cite{du15}}
\def\tbrefSpinnaker{\cite{Stromatias2013}\tablenote{Results extracted from 1st column of Table~III in~\cite{Stromatias2013}, infrastructure power assumed as \SI{11}{W} per board, cf. Figure~6 of~\cite{Stromatias2013}}}
\def\tbrefthiswork{this work\tablenote{at PL1 \SI{0.7}{V}}}

\Com{Needs update, Text from DVFS Paper}

power per synaptic event for neuromorphic benchmarks
coremark power for processor?
TOPS/W for DNN
Mixed Metric for hybrid approach (reduced TOPS/W, but more importantly the computed energy per synaptic event when using MAC as in Yexins proposals)

DNN table in addition to the neuromorphic table?

pick up on hybrid approach again, i.e. we achieve very high energy efficiency due to the accelerators, but still keep the flexibility of the processor


Although this work is focused on a dynamic power management technique for event-based digital neuromorphic systems, thereby not being directly comparable to other neuromorphic approaches, Tab.~\ref{tab:compare} compares the achieved energy consumptions also of different neuromorphic systems. 
For realistic comparison two metrics for synaptic energy are considered. First, the energy per synaptic event as in total energy divided by synaptic events processed across the system and second the incremental energy for one more synaptic event. These metrics are not scaled to the semiconductor technology, since completely different circuit approaches provide their optimal results in different technology nodes. For a fair comparison these metrics would have to be extracted from the same benchmark running on the different neuromorphic hardware systems \cite{diamond2016comparing}. 
We did not put memristor systems in the table, as the approach seems too different and no large-scale memristor systems have been reported. However, for comparison we would still name a few figures for memristor synapse arrays: Du et al.~\cite{du15} report measurements of \SI{4.7}{pJ} for potentiation/depression at a single synapse, but without the circuit overhead. Chakma et al.~\cite{chakma2018memristive} simulate memristors and CMOS neurons, reporting between 0.1 and \SI{10}{pJ/synaptic operation} for both learning and passive memristors, with additional \SI{10}{pJ/spike} for the CMOS neurons. Analog subthreshold systems \cite{Benjamin2014,qiao2015reconfigurable,Yu2012,moradi2017scalable} and mixed-signal systems \cite{Schmitt2017,mayr2016,noack14b} use analog circuits to mimic neural and synaptic behavior. Custom-digital neuromorphic chips \cite{merolla2014million,frenkel2018,Davies2018} use event based processing in custom non-processor units. They can be implemented in nanometer CMOS technologies and show low energy per synaptic event regarding total power in the same order of magnitude as the analog and mixed-signal approaches. 
Multi-processor based neuromorphic systems, such as this work, trade off much higher system flexibility due to software defined neuromorphic processing by two to three orders of magnitude higher energy consumption. However, the scaling of semiconductor technology together with dynamic power management techniques such as the proposed DVFS in this work reduces this gap. Compared to SpiNNaker approximately $10\t{x}$ reduction of neuron processing energy and PE energy per synaptic event is achieved. For our benchmarks on this work, as summarized in Tab.~\ref{tab:powermeas}, the application of DVFS results in 73\% total PE power reduction. The proposed technique is also applicable to custom-digital neuromorphic systems which operate in an event-driven fashion.


\setrowcolors{}
%Results table
\begin{table*}[htb]
  \begin{minipage}{0.97\textwidth}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \caption{Efficiency comparison of neuromorphic hardware systems}\label{tab:compare}
    \centering
    \footnotesize
    \begin{tabular}{llcccp{2.5cm}c} \toprule \setrowcolors{}
       System               & Reference           & Type                     & Techn.\ node & Neuron power      & E/SynEvent                                                                         & E/additional SynEvent \\
                            &                     &                          & [\si{nm}]    & [\si{nJ}/\si{ms}] & [\si{pJ}]                                                                          & [\si{pJ}]             \\ \midrule
       Neurogrid            & \tbrefNeurogrid{}   & analog sub-Vt            & 180          &                   & 119                                                                                & n.a.                  \\ % checked
       ROLLS                & \tbrefROLLS{}       & analog sub-Vt            & 180          &                   & n.a.                                                                               & 0.077                 \\ % checked, single synaptic event.
       HiAER-IFAT           & \tbrefHiAER{}       & analog sub-Vt            & 130          &                   & 50                                                                                 & n.a.                  \\ \midrule% checked
       cxQuad               & \tbrefcxQuad{}      & mixed-signal             & 180          &                   & 46                                                                                 & 0.134                 \\ % checked, incoming syn event is broadcast to 256 tgts
       BrainScales          & \tbrefBrainScales{} & mixed-signal accelerated & 180          &                   & 100                                                                                & n.a.                  \\ % checked
       Titan                & \tbrefTitan{}       & mixed-signal             & 28           &                   & 18                                                                                 & n.a.                  \\ \midrule
       TrueNorth            & \tbrefTrueNorth{}   & custom digital           & 28           &                   & 26                                                                                 & n.a.                  \\ % checked
       Odin                 & \tbrefOdin{}        & custom digital           & 28           &                   & 12.7                                                                               & 8.4                   \\ % checked
       Loihi                & \tbrefLoihi{}       & custom digital           & 14           & 0.052             & n.a.                                                                               & 23.6                  \\ \midrule % checked

       %BiFeO3 memristor    & \tbrefmemristor     &                          &              &                   &                                                                                    & 4.7                   \\ \midrule % checked
       SpiNNaker            & \tbrefSpinnaker{}   & MPSoC                    & 130          & 26                & 13300\tablenote{regarding PE power only} (19300) \tablenote{regarding total power} & 8000                  \\

       SpiNNaker2 prototype & \tbrefthiswork{}    & MPSoC                    & 28           & 2.19              & 1500 (4500)                                           & 450                   \\

      \bottomrule
      %thiswork: Use no benchmark but locally connected random network as in SpiNNAker1, at PL1 )0.70V).
    \end{tabular}
    \vspace{0.8ex}

    For all systems we report the best case with highest energy efficiency found in literature.  Note that results are not fully commensurable, especially for the metric considering total power, as different benchmarks are applied.
  \end{minipage}
\end{table*}


%Christian: I don't really understand the figures in the truenorth row. Merolla14 imho had incremental energy per synaptic event of \SI{45}{pJ/spike}, not absolute energy per spike of \SI{26}{pJ/spike}. I don't find the \SI{26}{pJ} value anywhere in the paper.
%Bernhard: The \SI{26}{pJ} are in the~\cite{merolla2014million} on page 671: "At the operating point where neurons fire on average at \SI{20}{Hz} and have 128 active synapses, the total measured power was \SI{72}{mW} (at \SI{0.775}{V} operating voltage), corresponding to \SI{26}{pJ} per synaptic event (considering total energy)."
%You probably refer to~\cite{merolla2011digital}, which indeed reports \SI{45}{pJ}/spike in the title.

%Why do we show this comparison table, and why so many systems?
%The conclusions to draw are the following:
%1. we are one order of magnitude better than SpiNNaker1
%2. Dedicated digital system (Truenorth, Loihi) are about 1 or 2 orders of magnitude more energy efficient.
%3. Large-Scale Analog systems (neurogrid, Brainscales) are not better than dedicated digital systems (when looking at the total power consumption) --> nicht belegt in Tabelle.
%4. Zürich's systems: cxQuad: \SI{46}{pJ} are not better than custom digital systems.


